COMMAND: Certifiable Open Measurable Mandates

Security mandates today are often in the form of checklists and are generally inflexible and slow to adapt to changing threats. This paper introduces an alternate approach called open mandates, which mandate that vendors must dedicate some amount of resources (e.g. system speed, energy, design cost, etc.) towards security but unlike checklist security does not prescribe specific controls that must be implemented. The goal of open mandates is to provide flexibility to vendors in implementing security controls that they see fit while requiring all vendors to commit to a certain level of security. In this paper, we first demonstrate the usefulness of open security mandates: for instance, we show that mandating 10% of resources towards security reduces defenders losses by 8% and forestalls attackers by 10%. We then show how open mandates can be implemented in practice. Specifically, we solve the problem of identifying a system's overhead due to security, a key problem towards making such an open mandate enforceable in practice. As examples we demonstrate our open mandate system -- COMMAND -- for two contemporary software hardening techniques and show that our methodology can predict security overheads to a very high degree of accuracy (<1% mean and median error) with low resource requirements. We also present experiments that quantify, in terms of dollars, how much end users value the performance lost to security, which help determine the costs of such a program. Taken together -- the usefulness of mandates, their enforceability, and their quantifiable costs -- make the case for an alternate resource-based mandate.

==> Makefile <==
PAPER	= main
TEX	= $(wildcard *.tex)
BIB	= $(PAPER).bib
FIG	= $(wildcard figures/*.*)
LATEX	= pdflatex -shell-escape
BIBTEX	= bibtex

.PHONY: all clean

all: $(PAPER).pdf

$(PAPER).bbl: $(BIB)
	$(LATEX)	$(PAPER)
	$(BIBTEX)	$(PAPER)

$(PAPER).pdf: $(PAPER).bbl $(TEX) $(FIG)
	$(LATEX)	$(PAPER)
	$(LATEX)	$(PAPER)

clean:
	$(RM) *.aux *.bbl *.blg *.log *.out $(PAPER).pdf

spellcheck:
	for i in *.tex; do \
    	aspell -c -t $$i ; \
	done

==> acknowledgement.tex <==
\section*{Acknowledgment}

==> background.tex <==
\section{Background}  \label{sec:back}
 
% Mandates in the realm of cybersecurity have not been a rare occurrence.
% Recently, they have been a regular occurrence from varied official sources, including executive orders, standards crafted by standards organizations, and legislation.


==> extension.tex <==
\section{ISA Extension}  \label{sec:extension}


\begin{itemize}
 
    \item Describe our hypothetical ISA extension.

\end{itemize}






==> framework.tex <==
\section{Framework} \label{sec:frame}

% % The goal here is to measure the amount of energy a system spends on security.
% Our framework is a set of general guidelines and principles that engineers can use to determine the amount of energy a system spends on security.

% TODO: What is the framework?

% \begin{itemize}
%     \item 
% \end{itemize}

% If we break a system down into its hardware components, then \textit{some} 
% For example, 

% \subsubsection{Attempt \#1: Easily Demarcated Hardware and Software}

% $$ \text{Security Effort} := \frac{E_s}{E_s + E_i}$$

% \subsubsection{Attempt \#2: Interference}

% We must use a function of the current microarchitectural state, and the security features currently being used

% We estimate the energy of security as 
% $$ E_{s, measurable} + E_{s, immeasurable}$$
% $$ = E_{s, measurable} + f(\text{state}, \text{features})$$
% The goal then becomes to find a suitably approximating function $f$.

% Software demarcation:
% SGX, MPX, etc.

% \subsection{Pitfall, Limitations, and Mitigations}

% \subsection{Implementing the Framework}

% We now describe three implementations of our Energy Monitor Framework.

% \subsubsection{Cost of a Context Switch}

% ASID
% Flushing?
% Cost of user/supervisor bit

% NOTES from book: 
% part of kernel is included in process virtual address spaces, so that context switches are less costly.
% enforcing limited access permissions  (rwx) 
% Pages cannot have r+w+x simultaneously. This is a security features, but presumeably causes no additional energy overhead. Just good design

% For example, if a core performs a context switch, a TLB without process ID bits will have to be flushed to ensure that no homonyms from the old context are accidentally treated as being part of the new context. 
% The second is to attach a process or address space ID to each
% virtual address whenever two addressed from different process might be compared, and then to
% track the process or address space ID in the translation caching structures as well. For example,
% as we discuss in Section 4.5.3, some TLBs (but not all) associate a process ID of some kind with
% each page table entry they cache, for exactly this reason.

% x86:
% r/w bit
% x bit
% u/s bit
% global bit (whether it needs to be invalidated upon a context switch)
% page table walk: each level also hold permission bits

% ASID in TLB means you don't have to flush on context switch

% Have to flush stale TLB entries (TLB shootdown, varies widely by architecture)

% Context Switch requirements not related to security, but still have to do:
% switching registers

% Have to switch to supervisor mode to handle context switch

% difference between isolation vs security?

% Multiple level TLBs

% \subsubsection{User Authentication Program}

% \subsubsection{Web Browser}

% \subsubsection{Pointer Authentication Codes}

==> mandate.tex <==
\section{Mandate}  \label{sec:mandate}

\subsection{Definition}

We would like to analyze the computer architectural impact of the government imposing a mandate as follows:

\textbf{Any organization operating in the jurisdiction of some government imposing this mandate must allocate x\% of their assets toward the improvement of the security of their products in terms of software and hardware. }

We argue that such a mandate is:
\begin{itemize}
	\item Reasonable to impose
	\item Enforceable
	\item Does not create a burden of implementation that is too large
	\item Likely to have a positive economic effect in the jurisdiction of the imposing government
\end{itemize}

\subsection{Reasonability}
We first begin to establish that this mandate is reasonable by drawing parallels to other industries in which such mandates have been adopted.
Take for example the car industry, in which the extreme environmental impact of automobiles has been curbed via government mandates that regulate emissions from automobiles.

\textbf{TODO} Can probably expand on these examples and cite

It is clear that in recent history, different countries have been devastated by a lack of security hygiene. 
Take for example the infamous SolarWinds hack in the United States, in which foreign powers infiltrated companies contracted by the United States government and were able to use this leverage to eventually breach US government entities.
Similarly, there was the shutdown of the Colonial gasoline pipeline in the southeastern United States due to a ransomware attack.
Though both of these attacks were not directed specifically at the government of the United States, they still had an incredible impact on the infrastructure that the United States government relies on to function.
The assets of companies operating within a government's jurisdiction have fundamental ties to the both the economic well-being of a nation and the security of the government itself.
This, we argue, is an extraordinarily compelling reason for a government to issue a mandate such as the one outlined above. 

\subsection{Enforcement}
Furthering the analogy to the car industry, there are regulatory bodies in place to audit both the designs of car manufacturers as well as individual manufactured automobiles.
Our mandate requires organizations to dedicate some amount of their assets towards security.
We propose that some regulatory body, be it affiliated with government imposing the mandate or a third party organization, be put in place to audit organizations that are subject to the mandate.

\subsection{Implementation and Economic Effect}
We devote the next sections to showing how our mandate would be implemented and demonstrating the positive economic impact of implementing such a mandate.

% % A proposal for a mandate: We propose mandating that system must use a certain percentage of their energy towards achieving security.

% % Why energy? Because it's the currency of computation. 
% % (Give a list of other ways hardware security could be mandated and why they fail)

% % What is our mandate trying to fix?
% % Our proposed mandate then needs to address these four reasons of market inefficiency
% An ideal mandate should provide society with a higher level of security at a lower overall cost. 
% This can be achieved if the mandate addresses and corrects the four identified reasons for security marketplace inefficiencies. 
% However, while these conditions are necessary, they are not sufficient.
% In order for the benefits of a mandate to outweigh costs, a mandate should also:
% % In addition, an ideal mandate should also follow a few additional constraints.
% % In particular, an ideal mandate should:
% \begin{itemize}
%     \item Cover insecurity at both the hardware and software levels. This is essential, because security is a full-system property: Since the security of a system typically reduces to the security of its weakest link, widespread improvements to security will require improvements to all levels of the computing systems stack.
%     % \item Improve security both during the design of systems (including hardware, software, and configuration) and during operation. % we achieve this by mandating recurring and non-recurring costs.
%     \item Improve the security of systems at all stages of their lifecycle, from development and manufacturing to configuration and operation.
%     \item Be permissive enough to not be unreasonably burdensome or constrain innovation.
%     \item Be enforceable. That is, it should be relatively easy to determine whether or not a mandate is being followed. 
% \end{itemize}

% Using these constraints as our guidelines, we propose the following mandate:

% \noindent
% \framebox{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{\itshape\textit{
%     Computer systems must make an honest effort towards security.
%     This can be enforced in a twofold manner:
%     First, systems must be designed to be secure.
%     Since defining ``secure design'' is such an elusive and immeasurable requirement, we instead mandate secure design by proxy:
%     Namely, companies that design and sell computer system products (including both hardware and software) must dedicate a fixed percentage of development and integration costs towards security.
%     Second, systems must be operated in a secure manner.
%     Since defining ``secure operation'' is such an elusive and immeasurable requirement, we instead mandate secure operation by proxy:
%     Namely, systems must dedicate a fixed percentage of their overall energy consumption towards security.
% }}}

% % Explain why this mandate meets our requirements...
% % We now examine how this mandate addresses the four 

% % Our mandate fixes the market failing
% \

% This proposal stands to fix the three identified failings of the security marketplace. First, the mandate nudges economies away from tragedies of the commons: Requiring systems to adhere to a baseline effort of security prevents users and companies from ``free-riding'' or shirking their communal responsibility to uphold security. 
% For example, the mandate on secure design
% % ---particularly the requirement that chip makers dedicate a percentage of silicon area towards security---
% prevents systems designers from trading off security features for higher performance. 
% This prevents the marketplace, driven by large corporate buyers generally seeking performance over security, from acting against its own self interest and ensures that no product undercuts its competition by shirking its responsibility to provide security.

% Second, our mandate addresses problems of misaligned incentives. 
% % Mandating that the companies who protect data must 
% % Companies who build systems to protect data must make an honest effort in protecting their data. Likewise, mandated operational security 
% Companies entrusted to protect sensitive information must make an honest effort in protecting their data. This is addressed both by the secure design portion of the mandate (ensuring that the necessary safeguards are in place) and the secure operation of the mandate (ensuring that once the safeguards are in place, they are actually being used). This fixes the problem of asymmetric information between consumers and companies: Security-illiterate consumers won't need to make informed decisions on the security practices of various companies, since each company will be required to maintain some minimum standard. As an analogy, consumers in a grocery store don't need to inspect every piece of produce to determine if it's safe to eat---FDA regulations require produce to meet a  minimum standard that absolves consumers the burden of making informed decisions themselves.

% And third, the mandate prevents the security marketplace from devolving into a marketplace for ``lemons''. As previously stated, a contributing factor to insecurity is the information asymmetry between systems designers and systems users. Since most users cannot distinguish between a secure product and an insecure product, an unregulated market will tend towards overproducing insecure products. The mandate rectifies this problem:
% Requiring systems designers to include security as a design constraint means that products are better at being secure, whether the end user is aware of this or not.


% % The non-recurring aspect of the mandate addresses issues of 
% % Likewise, the recurring aspect of the mandate addresses issues of insecure operation. Under the mandate, a server farm couldn't lower security effort during peak times

% % Our mandate also follows the other constraints:
% Economics aside, our mandate is only practical if it also adheres to our four identified qualities of a good mandate. 
% Of the four, our mandate clearly follows the first three. 
% First, it is clear that a mandate on all aspects of computer systems naturally covers both hardware and software.
% Similarly, mandating effort at the design and operation stages of a products usage covers all aspects of a product's lifecycle. 
% And third, while the mandate inevitably introduces overhead and undeniably restrictive on how systems can be designed and operated, we feel that this burden is not unreasonable, given the potential benefits. 

% It is not so obvious how our mandate can follow our fourth requirement, namely that it should be enforceable. We examine the two portions of the mandate independently.

% \subsection{Enforcing Mandatory Budget Spending}

% % Largely out of scope for this paper.
% Our mandate's first major requirement is that systems must be designed with security in mind.
% This requirement ensures that companies are dedicating an appropriate amount of effort towards security when creating their products.
% We concede that design ``effort'' can take many different forms, each of which may be valid approaches towards meeting this requirement.
% For example, demonstrating that a percentage of a company's operational budget is spent on developer training and security education could be a valid expense that contributes towards ``effort''.
% To ensure that designs themselves make sufficient security tradeoffs, it may also be necessary to extend this requirement to domain specific requirements, such as computer chips dedicating a certain percentage of silicon area towards security features. 
% Regardless, implementing this portion of the mandate is an achievable but largely non-technical problem.
% In this paper, we choose to focus on the more technical features of the mandate (particularly measuring the energy cost of security), and leave the details of this portion of the mandate for the lawyers to figure out.

% \subsection{Enforcing Mandatory Energy Spending}

% % The precise scope of this paper.
% Our mandate's second major requirement is that systems must be operated with security in mind.
% % While this may seem, upon first glance, like a mandate on user behavior, our choice of mandating energy consumption 
% Upon first glance this may seem like an attempt to mandate user behavior.  
% On the contrary, we acknowledge that expecting all computer users to have a satisfactory knowledge of secure computer operation is extremely unrealistic.
% For this reason, our mandate instead intends to remove the user from the loop entirely, and instead dictate that ``secure operation'' is determined by the amount of effort a system is dedicating towards secure operation. 
% As stated previously, this is achieved by proxy:
% To determine security ``effort'', we will consider the percentage of system energy spent of security.

% (Argue why this is acceptable)

% This step is very non-trivial and fraught with pitfalls, which is why we introduce a framework for identifying the percentage of total energy dedicated towards security in \cref{sec:frame}.


% % We now present a more formal definition of our proposed mandate.

% % Our proposed mandate consists of 

% % \subsection{Other Mandates}

% % \begin{itemize}
% %     \item \textit{Mandatory Security Literacy}
% %     \item \textit{Mandatory Professional Certification}
% %     \item \textit{Mandatory Budget Expenditures}
% %     \item \textit{Mandatory Design Review}
% %     \item \textit{Mandatory Penetration Testing}
% %     \item \textit{Harsher Punishments for Insecurity}
% %     \item \textit{Catch the Criminals}
% %     \item \textit{Mandatory Security Insurance}
% %     \item \textit{Mandatory Standards Compliance}
% % \end{itemize}



==> model.tex <==

\begin{table*}[]
\centering
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Parameter}                         & \textbf{Definition}                                                                              \\ \hline
    \scriptsize{ATTACKERS}                     & Number of attackers compared to defenders, as a percentage                                          \\ \hline
    \scriptsize{PAYOFF}                            & Max percentage of defender assets that can be taken in an attack                                     \\ \hline
    \scriptsize{INVESTMENT}                   & Percentage of defender assets that are spent on security measures                               \\ \hline
    \scriptsize{EFFECTIVENESS} & Percentage of INVESTMENT by which the cost to attack a defender increases           \\ \hline
    \scriptsize{INEQUALITY}                       & Fraction by which defender wealth distribution is scaled to create attacker wealth distribution \\ \hline
    \scriptsize{SUCCESS}    & Initial percentage of defender assets that count toward the cost to attack a defender \\ \hline
    \end{tabular}
    \caption{Parameters of our Monte-Carlo model}
    \label{table:params}
\end{table*}

\section{Are Mandates Useful?}\label{sec:model}

In this section we provide the details of our modeling process that gave us the statistics we discussed in Section~\ref{sec:motivate}.
In order to construct the model we discussed in the previous section, we chose to use Monte Carlo simulation techniques as a proxy for an existence proof of economic conditions under which a mandate would be beneficial. 
Here we define ``beneficial'' as 1) decreasing the amount of assets that good actors lose to malicious actors and 2) lengthening the amount of time necessary for malicious actors to steal the assets of good actors.
Our simulations model the following scenario:

\subsection{Model Construction}

\subsubsection{Setup and Initialization}
\begin{itemize}
    \item Players are split into a group of \textit{attackers} and a group of \textit{defenders}. There cannot be more attackers than defenders.
    \item Defenders are initialized with an approximately lognormal distribution of \textit{assets} drawn from global data generated by Credit Suisse~\cite{suisse} along with a \textit{cost to attack}, which can be interpreted as a threshold (in terms of assets) that an attacker must pay to take a portion of a defender's assets.
    \item Attackers are assumed to be on average less wealthy than defenders: Assets of attackers are determined by scaling the defenders' lognormal distribution of assets by a percentage, which we label \textit{inequality}.
    \item Attackers have perfect information about defender assets, but defenders do not have perfect information about attackers. This models an information asymmetry.
    \item Our model contains 6 parameters that are shown in Table~\ref{table:params}. 
Each parameter can be thought of as a percentage, with real values [0, 1].
\end{itemize}

This information is required to establish the initial conditions of each scenario for our model. 
We now describe the rules in order to carry out a simulation.

\subsubsection{Rules}

For each iteration of the simulation, the following steps are performed:

\begin{enumerate}

\item Each member $d$ of the defenders $D$ is associated its assets $d.assets$, and its cost to attack $d.cost$. 

\item Each member $a$ of the attackers $A$ is associated with a number representing its assets $a.assets$ and is assigned its probability of attacking successfully $p_{success}$.

\item Each attacker $a$ is paired with a defender $d$.

\item Each $a$ ``fights'' the $d$ it has been paired with in the following way:
The attacker computes its expected earnings given the $d$ it has been paired with and $p_{success}$

\item Each $a$ then checks whether $a.expected\_earnings < d.cost$ and if $d.cost < a.assets$.
If these conditions are met, $a$ performs an attack on $d$. $a$ wins with probability $p_{success}$.

\item Attackers are punished via a loss of assets if their attack fails, and if the attack fails $d.cost$ is subtracted from $a.assets$.

\item Any $d$ s.t. $d.assets \leq 0$ is then removed from the game following the fight, before the next iteration of the game takes place, and the next iteration carries out starting at step 1 above.

\end{enumerate}

We obtained our value for $p_{success}$ from a report analyzing ransomware incidents across a variety of different economic sectors.
We see that on average, 39\% of ransomware attacks are successful with a standard deviation of 6.2\% across the included sectors~\cite{sophos}.
We use these values to create a normal distribution and select a value from this distribution when an attack is carried out during each iteration.
An attackers' expected earnings are computed using the following equation:
\[ a.expected\_earnings~=~d.assets~*~\mathrm{PAYOFF}~*~p_{success} \]

\subsubsection{Termination}
Simulations terminate under three possible conditions:

\begin{enumerate}

\item $\forall d \in D$, $d.assets \leq 0$.

\item The simulation converges, where given two successive iterations of the simulation $i$ and $i+1$, ``convergence'' is defined as meeting the following condition for $\geq \delta$ iterations:  
 \[ \sum_{i+1} d.assets - \sum_{i} d.assets  \leq \epsilon\]

\item A set maximum number of iterations is reached, although we ran our simulations with a maximum of 10,000 iterations and never reached this threshold.
\end{enumerate} 

In our simulations, $\epsilon = \$100$ and $\delta = 50$ iterations.
Given that these simulations are not pinned to a specific timescale, we justify our choices of $\epsilon$ and $\delta$ via empirical observation.

%\begin{figure*}[h]
%    \centering
%    \begin{subfigure}[t]{0.3\textwidth}
%        \centering
%        \includegraphics[width=\columnwidth]{sim_2.png}
%        \caption{
%            A game with \texttt{PERCENT\_EVIL}=0.2, \texttt{PAYOFF}=0.7, \texttt{WEALTH\_GAP}=0.3, \texttt{ATTACK\_COST\_CONVERSION\_RATE}=0.2, and \texttt{SEC\_INVESTMENT}=0.0.
%            % The game stabilizes at around 300 iterations of the simulation, with the Attackers collectively winning a sizeable portion of the Defenders' initial assets.
%            }
%        \label{fig:sim:1}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}[t]{0.3\textwidth}
%        \includegraphics[width=\hsize]{sim_3.png}
%        \caption{
%            A game with \texttt{PERCENT\_EVIL}=0.5, \texttt{PAYOFF}=0.8, \texttt{WEALTH\_GAP}=0.7, \texttt{SEC\_INVESTMENT\_CONVERSION\_RATE}=0.1, \texttt{ATTACK\_COST\_CONVERSION\_RATE}=0.1, and \texttt{SEC\_INVESTMENT}=0.2.
%            % This configuration of parameters results in the Attackers looting essentially all of the Defenders' wealth.
%        }
%        \label{fig:sim:2}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}[t]{0.3\textwidth}
%        \includegraphics[width=\hsize]{sim_4.png}
%        \caption{
%            The same parameters as in (b), but with \texttt{PAYOFF}=0.2. 
%            % With a lower payoff scaling factor, the incentives for attacking are less and the game converges nearly immediately into a stalemate, with Defenders losing essentially no assets to the Attackers. 
%        }
%        \label{fig:sim:3}
%    \end{subfigure}
%    \caption{
%        Example system behavior for a variety of different input configurations.
%        Some games like (a) see a moderate transfer of wealth between Defenders and Attackers while other games like (b) see the Attackers loot essentially all of the Defenders' wealth.
%        Still other games like (c) see a near-instant stalemate, with virtually no wealth transferred from Defenders to Attackers. 
%    }
%    \label{fig:cdf2}
%\end{figure*}


==> results.tex <==
\section{Results}  \label{sec:res}

These are the ranges of parameters we thought to be reasonable:

\begin{itemize}
    \item: SEC\_INVESTMENT from 0.0 to 1.0 at increments of 0.1
    \item etc
\end{itemize}

Games can be described by six datapoints:
\begin{itemize}
    \item Blue team initial assets
    \item Blue team final assets
    \item Red team initial assets
    \item Red team final assets
    \item Crossover point
    \item Number of iterations for the game to converge
\end{itemize}

We then compute the ratio of blue initial to blue final assets.

Another metric we look at is the rate of loss.
All these being equal, it is preferable that Defenders lose their assets more slowly.

For each set of parameters, we find the mandate that maximizes Defenders' final assets.
Here are some plots that demonstrate what levels of SEC\_INVESTMENT are good for various parameters.
% \subsection{User Authentication Program}

% \subsection{Web Browser}

% \subsection{Pointer Authentication Codes}

==> sensitivity.tex <==
\subsection{Results} \label{sec:sens}
In this section we perform a detailed analysis of the results of our Monte-Carlo simulations and use them to summarize why a mandate would be beneficial to implement given the current state of the world we live in.

\subsection{Full Simulation Results}
Our results show (see Figure ~\ref{fig:cdf}) that upon imposing a 10\% investment in security, 8\% more of the scenarios in our model then experience only the losses of the security investment and do not have their assets plundered by attackers.
This trend then continues with diminishing returns as we increase the percentage of assets required to be invested in security, with a 20\% mandate adding another 7\% of scenarios, a 30\% mandate adding another 6\%, and so forth.
This creates a new question: does the world state that we are in correspond to the space where a mandate is useful or not?
This question can be answered with a simple argument---namely that to be in the space where mandates are not useful would imply that parties associated with ``defenders'' in our modeling are not losing their assets.
This is undoubtedly false, as we have seen cyber-incident after cyber-incident cost governments, companies, and individuals countless assets, especially in recent years.
Given these observations, it is clear that the world currently lies within the parameter space in which a mandate would be useful---these ``useful'' states correspond in our model to scenarios in which attackers are continually able to rob defenders of their assets with little fear of being caught.

Beyond the most desirable outcome for an individual ``defender'', losing no assets, we would additionally like to establish whether or not mandates can stem cumulative losses over time.
In this respect we classified the negative outcomes of our model into two categories: 1) simulations under which the parameters led to the complete loss of all defender assets, and 2) simulations under which the parameters led to an ``equilibrium'' in which after the protracted loss of assets by many defenders, the losses eventually halted asymptotically over time.

In our simulations, the first outcome occurred in 1\% of suboptimal scenarios (Figure ~\ref{fig:total_loss}), while the vast majority were associated with the second.
Even in the worst case of complete loss of defender assets, we see that a mandate increased the amount of time before this happened, and in the slightly better case that only some defenders lost assets, we can see that the rate at which defenders lost assets reliably decreased with an increased mandate for investment, which we can see displayed in Figure ~\ref{fig:loss_rates}.

\begin{table}[h!]
\centering
\begin{tabular}{| l | c | } \hline
	\textbf{Parameter} & \textbf{Expected Value} \\\hline
	\scriptsize{ATTACKERS} & 0.5 \\\hline
	\scriptsize{PAYOFF} & 0.8 \\\hline
        \scriptsize{INVESTMENT} & 0.2 \\\hline
        \scriptsize{EFFECTIVENESS} & 0.5 \\\hline
        \scriptsize{INEQUALITY} & 0.5 \\\hline
        \scriptsize{SUCCESS} & 0.3 \\\hline
\end{tabular}
\caption{ Expected values of Monte-Carlo parameters}
\label{table:expected}
\end{table}

\subsection{Determining Useful Model Configurations}
We define a ``useful'' configuration of parameters for our model to describe the set of parameters when a full run of the simulation in which the end result differs from the initial system conditions after more than the minimum number of iterations have passed.
In complement, a configuration of parameters that is not ``useful'' implies that for a set of given initial conditions, the attackers are unable to take any assets from the defenders and the simulation terminates at the minimum possible threshold for simulation convergence $\delta$.

The histogram depicted in Figure~\ref{fig:hist_mc} displays the distribution of parameter values for useful parameter sets.
From them we can make several observations regarding the model parameters:

\begin{itemize}

\item Attackers and their relative inequality have little (if any) effect on whether or not the model will produce a situation in which the global state would benefit from a mandate. The ``useful'' simulations are distributed approximately equally throughout the possible values for these model parameters--in fact, so evenly that in Figure~\ref{fig:hist_mc} the two lines for the ATTACKERS and INEQUALITY parameters are indistinguishable at the scale that we present the figure.

\item Attackers are favored heavily by lower values of SUCCESS as well as lower INVESTMENTS among parameter sets that are receptive to the introduction of a mandate. This makes sense, as this implies that the attackers have their greatest successes when a) there is low investment in security and/or b) there is little to no initial security investment

\item Attackers are favored mildly by lower values of EFFECTIVENESS, which implies that although clearly an effective investment in security would be preferred to an ineffective investment, it is indeed secondary to having such an investment, within the bounds of reason.

\item Attackers are favored heavily by higher values of PAYOFF. This makes sense, as an increased PAYOFF allows for attackers to steal larger and larger portions of the defenders' assets. We note that for PAYOFF $< 0.2$, attackers are unable to succeed in any circumstance.

\end{itemize}

\subsection{Maximum Utility Estimation}
We wanted to further analyze the space of useful parameter sets.
In order to do this, we calculated the expected value for each parameter \textit{over all useful simulations}, shown in Table~\ref{table:expected} and from the configuration with these parameter values, swept each model parameter relative to this parameter set for different values of the mandate investment.
We found that a substantial portion of these results were successfully encapsulated by Figure~\ref{fig:cdf}, but that graphs for a subset of the parameters (see Figure~\ref{fig:sweeps}) provided further insights into the workings of useful parameter sets.
%Graphically we can see that each per-mandate curve in Figure~\ref{fig:cdf} could be represented by a bimodal distribution, with an initial jump in the percentage of simulations covered by the neighborhood surrounding the initial mandate investment percentage and another, slighter jump from 90 to 100\%, suggesting another small cluster of simulation parameter sets in which a group of defenders loses most or all of their assets to the attackers.
%These bimodal characteristics stay as the mandate investment is increased, and the beginning and end clusters appear to gradually flatten out with an increase in the mandated investment.
%Following these observations we concluded that it would be of maximum utility to perform a sweep through the parameter values of each parameter with respect to different values of the mandated security investment with the goal of best determining the effects of the mandate in terms of the other simulation parameters.
%The results of this sweep for the other simulation parameters can be partially observed through Figure~\ref{fig:sweeps}, which detail full sweeps of 2 of the remaining 5 model parameters with respect to the security investment.

From these figures we are able to make the following conclusions w.r.t. the parameters of the model:

\begin{itemize}

\item EFFECTIVENESS, displayed in Figure~\ref{fig:sicr_sweep}, which represents the effectiveness of a given fixed INVESTMENT, no longer matters by the time INVESTMENT = 0.5. 
For the range $0.2 \leq \mathrm{INVESTMENT} < 0.5$, an increasing EFFECTIVENESS reliably decreases defender losses. 
Once the INVESTMENT is increased beyond these levels, it dominates the loss.
We can observe given this figure that different mandates are optimal given different values for EFFECTIVENESS, which implies that an expectation of how effectively defenders will manage their assets in turn governs which mandate might be the most effective.
For example, for $0.1 \leq \mathrm{EFFECTIVENESS} < 0.3$, a 40\% mandate minimizes total relative loss, while for $0.3 \leq \mathrm{EFFECTIVENESS} < 0.8$ a 30\% mandate minimizes the loss. 
If maximum effectiveness is enabled, a 20\% mandate becomes optimal.

\item As INVESTMENT is increased, attackers require a larger PAYOFF, displayed in Figure~\ref{fig:payoff_sweep}, for incentivization to attack.
Similarly to the previous sweep in Figure~\ref{fig:sicr_sweep}, we see that for INVESTMENT$\geq 0.4$, losses from defenders are dominated by the investment itself and the PAYOFF is effectively ``saturated'' and no longer meaningfully affects the outcome of the simulation.
Cross-referencing with Figure~\ref{fig:hist_mc}, we recall that for values under 0.2, there are no useful simulation outcomes and see that the lowest threshold for PAYOFF is at 0.4, when there is zero mandated investment.

\item We note that the results for the ATTACKERS parameter and INEQUALITY parameter do not change the total relative loss of assets experienced by defenders inherently. However, both do display that relative defender loss decreases with an increasing INVESTMENT. This information can be inferred without explicitly including these graphs, so we have chosen to omit them, along with the SUCCESS parameter.

\end{itemize}

\subsection{Summary}
Given our Monte-Carlo style model for an attack-defend scenario based on the real-world statistics for ransomware, we have demonstrated the tangible effects of a mandatory security investment by corporate, individual, and government ``defenders''.

In addition to the clear net benefits for defenders in terms of relative losses over time, the model emphasizes that it is the defender's job to allocate the security investment as wisely as possible (EFFECTIVENESS) as well as consider its security policies related to their assets as a whole (SUCCESS).
We have shown how the model indicates that just over one third of global scenarios can benefit from a mandate and that we currently reside in this space of parameters.
We have observed how the different parameters of the model were constructed and how they interact with each other in terms of establishing improvement via a mandated security investment.
In addition, we would like to acknowledge the existence of ``black swan'' events, or unexpected high-impact events that happen with a predictable frequency~\cite{swans}. This is a category of events which could and should be included in future work with respect to the modeling in this work.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.6]{hist_mc.pdf}
    \caption{Histogram of useful Monte-Carlo simulation parameters}
    \label{fig:hist_mc}
\end{figure}
    
\begin{figure*}
    \begin{subfigure}[t]{0.5\textwidth}
        \includegraphics[width=\columnwidth]{SICR_inclusive.pdf}
        \caption{Sweeping EFFECTIVENESS parameter relative to assets invested in a mandate}
        \label{fig:sicr_sweep}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.3\textwidth}
%        \includegraphics[width=\columnwidth]{ACCR.pdf}
%        \caption{Sweeping conversion rate between initial defender assets and cost to attack defenders relative to assets invested in a mandate}
%        \label{fig:accr_sweep}
    \end{subfigure}
    \begin{subfigure}[t]{0.5\textwidth}
        \includegraphics[width=\columnwidth]{PAYOFF_inclusive.pdf}
        \caption{Sweeping attacker bounties relative to a mandated investment}
        \label{fig:payoff_sweep}
    \end{subfigure}
%    \hfill
%    \begin{subfigure}[t]{0.3\textwidth}
%        \includegraphics[width=\columnwidth]{PERCENT_EVIL.pdf}
%        \caption{Sweeping red team size relative to assets invested in a mandate}
%        \label{fig:pevil_sweep}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.3\textwidth}
%        \includegraphics[width=\columnwidth]{WEALTH_GAP.pdf}
%        \caption{Sweeping red team wealth relative to assets invested in a mandate}
%        \label{fig:wgap_sweep}
%    \end{subfigure}
	  \caption{Sweeping two of the six simulation parameters relative to the default configuration shown in Table~\ref{table:expected}}
	  \label{fig:sweeps}
\end{figure*}




==> taxonomy.tex <==
\section{Systems-Level Mandates and Defense Taxonomy}  \label{sec:taxonomy}

% Section on why a taxonomy is needed
% 

% Previous section is an existence proof for mandate spending security.
% But it's really general---``spending'' increases ``security''---these are not easily transferrable to the real world.
% Particularly that security can be represented as a single scalar value.
% The model also ignores the fact that this is more than just self-defense:
% Companies make products that other people use, and so they aren't always properly incentivized to pay for security since they don't internalize the costs.
The above simulations presents a simplified model of the dynamics between attackers and defenders.
From the conclusions, one might be tempted to think that the takeaway argument is that companies and organizations should be mandated to invest in their own security posture.
This, however, is \textit{not} the argument we wish to present.
As noted, it necessarily makes some simplifying assumptions about the state of the world, such as by representing overall individual security as a scalar value and by excluding network effects and the interdependence of security between defenders.
% Rather, we interpret the model as a practical example of why 
Therefore, the takeaway we wish to impart on the reader is that spending resources on security can result in better outcomes for the defenders.
In particular, we stress that the  scalar ``security'' level of a defender is a crude approximation of the real world, where security is a complex, unknown function with many inputs.
% There is a right level of security investment, we just don't know what it is.

Given that security is a full-system property, this means that security investment must be applied at all levels of the technology stack.
% And in areas where incentives do not lend well to investment, this means that we need mandates.
% And in areas where incentives do not 
However, as discussed in the introduction, security is under-invested at the systems and architecture level because the costs of insecurity are not internalized by vendors and information asymmetry between vendor and consumer prevents free markets from determining how much this investment should be.
The consequence, as suggested by the Monte Carlo simulations, is that security is in a suboptimal state, and that the overall costs of insecurity might be lower if product vendors were nudged to increase security investment in their products.\footnote{whew....gonna take a bit more to defend this line.};
This suboptimality might be overcome with mandated security investment at the systems and architecture levels of the technology stack.
\textit{But at the systems and architectural level, how can a government or regulator apply a mandate without devolving into checklist security?}

% So this is not just about organizational spending.
% The ``spending'' needs to be at all layers of the stack.
% \textbf{Security is a full-system property, so all parts of the system need to be putting forth effort towards security.}
% Same with fire safety---we don't just mandate how people should protect their own homes/business, but we also mandate products that are made for other people to use (e.g. you can't make a couch out of super flammable materials).
% This is a big challenge then, to keep in line with the spirit of the mandate (let companies decide how to secure their products) while also being actionable.
% \textbf{How does a system ``spend'' on security in a measurable or enforceable way?}
% Obviously systems can make tradeoffs for security (power, performance, area, e.g.) but ---.
% We need a proxy.
% Let's use performance as the metric of interest, since it is ultimately the currency of computing--All other factors can be converted to/from performance in one sense or another.

First, we point out an obvious but important fact:
System designers build systems but users are the ones who actually use them.
The nuance here is that an investment in security cannot take place solely during system design and integration since products have an ongoing lifespan.
Investment in security must be an ongoing process, yet at the same time is the responsibility of the system integrator to implement.
So, given a mandate to invest in security, what does it mean for a system to ``spend'' on security after it has already been purchased?
We propose the following:
\textbf{A systems- or architectural-level mandate to invest in security should be in terms of the currency of systems and architecture: performance.}
% In other words, a security investment mandate at the systems or architectural level should be as written as follows:
A mandate at the systems or architectural level should then be written as follows:
\textbf{Systems should dedicate some amount of performance towards security.}


% Any reader well-versed in the complexity of modern systems should immediately 
% Implementing such a mandate presents a tremendous number of truly challenging problems (both technical and non-technical) but the primary challenge is to measure how much performance a system is dedicating towards security in the first place.
% % So, the mandate becomes, ``Prodcuts should spend a certain amount of their performance on security''.
% % THIS IS NOT A TRIVIAL THING TO DO.
% % Companies are (rationally) going to want to avoid over-paying for security----how do we make sure they don't underpay?
% Despite all these difficulties, we assure the reader that a path forward is possible as demonstrated in Section~\ref{}.

The idea of a system ``paying'' for security in terms of performance is a nuanced and fraught with challenges because there are many different ways a system can dedicate performance towards security.
To reason about the ways a system can pay for security, we find it useful to define a taxonomy of defenses and how and where they ``pay'' for security.
We identify four dimensions along which a defense can be classified.


% To reason about how a system can ``pay'' for security in terms of performance, we need to first identify a taxonomy of system-level security defenses so that we know how a system can pay in the first place.
% I.e. a taxonomy of where and how security comsumes performance.
% We identify four dimensions along with a defense can be classified.

% This section needs an introduction and needs to explain why such a taxonomy is needed when discussing a security-performance mandate

% \textbf{Static vs. Dynamic}
\textbf{One-time vs. Always-on}---Defenses exist along a spectrum of how often they incur a cost to system performance.
At one end of the spectrum are \textit{one-time} costs, which (as the name implies) are incurred only once, and are then amortized over the course of a products' lifetime.
Examples include the cost of installing a device firewall or the overhead of prompting a user to pick a secure password, since these are steps that (in theory) only happen once and only cost performance (or its counterpart, usability) only once.
\textit{Intermittent} defenses cost performance only when they are applied, such as system-wide malware scans, which consume system resources but only during use.
Finally, at the other end of the spectrum, \textit{always-on} defenses come at a cost to performance for as long as the system or program is being used.
For example, the cost of communicating over an encrypted channel always incurs the cost of encryption and decryption, which is never amortized across usage.
Another common example is the cost of applying binary hardening techniques during program compilation and runtime:
 defenses protect programs from certain memory safety exploits but also cause a consistent and continuous loss of program performance. 

% In the implementation of our mandate, there is first a clear demarcation between what we consider to be ``static" and ``dynamic" overheads for putting different security mechanisms in place.
% ``Static" overheads are represented by one-time-costs with respect to an improvement of security hygiene, such as a company purchasing 2FA tokens for its employees or the conversion of some software application from a memory-unsafe language (e.g. C, C++) to a memory-safe language (e.g. Rust, Go). 
% As the overheads necessary to put a ``static" security mechanism in place are a one-time-cost that is then amortized over all future time, they can be viewed solely in terms of a financial investment in security without any dimension of depreciation of performance, power, or energy consumption.
% We use the term ``dynamic" to describe security measures that have a continual cost, typically systemic changes that will introduce a ``fee" on some performance metric over time.

\textbf{Dedicated vs. Non-dedicated}---Defenses can be classified by how dedicated or focused on security they are.
% Another dimension on which we can classify security features is whether they are targeted or non-targeted. 
% Modern systems have elements of security baked into nearly all components at all layers of the hardware-software stack.
% This does not mean, however, that all such components are strictly security features.
For example, consider virtual memory, which enables program sandboxing and isolation and also enables further defenses like non-executable stacks.
% It allows systems to place programs in virtual sandboxes of memory space and prevents potentially malicious programs from reading or writing in the address spaces the kernel or other co-located programs.
% Virtual memory also allows systems to assign permissions to memory pages, enabling further security features like non-executable stacks.
However, it would be a mistake to claim that virtual memory is solely a security technique, since it has many non-security benefits, like enabling program portability between devices.
Thus we classify virtual memory as a \textit{non-dedicated} security defense, since its benefits are not confined to security alone.
Additional examples of non-dedicated defenses include other isolation and virtualization techniques (e.g. using virtual machines on shared cloud servers protects users from each other but also enables useful operations like live migration) as well as the use of high-level programming languages (which may provide memory safety but also give programmers access to productivity-increasing high level language constructs and objects).
In contrast, \textit{dedicated} defenses improve security and achieve nothing else.
One such example is Address Space Layout Randomization (ASLR), which offers no benefit except making it harder for attackers to exploit memory safety vulnerabilities.


\textbf{Hardware vs. Software}---Defenses can be categorized by where in the hardware-software stack they are implemented.
% Pure hardware defenses 
Some defenses \textit{must} be implemented in hardware (e.g. the presence of a supervisor bit) while others may be implemented in hardware for performance reasons alone (e.g. on-chip AES accelerators).
Some hardware-backed defenses span the hardware-software divide (such as machine instructions that support locking).
Other defenses may be entirely implemented in software (such as system-wide malware scans or running programs with Address Sanitizer).
% can be independent of performance

% \subsection{Overhead Cost}


% HW can be lower cost

\textbf{Discrete vs. Diffuse}---The last dimension we consider is how easy it is to identify when and where security is costing performance.
% This dimension may seem similar to the one-time vs. continuous dimension.
%  whether defenses are \textit{discrete} or \textit{diffuse}.
% A \textit{discrete} defense costs performance in clear and measurable ways.
To illustrate this point, consider Intel's Software Guard Extensions (SGX), a set of ISA extensions that allow programmers to heighten the security of given  memory regions (called enclaves) via explicit calls to SGX software routines.
% The use of SGX requires programmers to explicitly declare when and where SGX operations are to be used.
Since SGX operations are also ``dedicated'' security operations (see above), we can conclude that all CPU cycles spent on SGX operations are contributing to security of the system.
Measuring the overhead of SGX is thus equivalent to measuring when SGX is being used, and is hence easy to accomplish.
We call such defenses \textit{discrete} since there is a well-established mechanism for determining when the defense is costing performance.
In contrast, a \textit{diffuse} defense does not have such clearly delineated markers of when a defense is or isn't costing performance.
For example, a compiler-based defense that increases binary size may put additional pressure of system caches, which can indirectly degrade performance.
The cost of this defense is then diffuse because it is not trivial to delineate when and where the defense introduces overhead.
Traditionally, the only method of measuring the overhead of such a defense is to run benchmark programs with and without the defense employed and comparing the runtime difference.

% % Another dimension that we describe is to label security practices as either \textit{discrete} or \textit{diffuse}. 
% A discrete security mechanism can be clearly portioned into sections representing security functionality and sections that are not relevant to security functionality by any party that implements the mechanism.
 
% Take for instance the Intel SGX system, encompassing both the hardware modifications necessary for its functionality, the changes to the ISA allowing for use of this new hardware, and the software infrastructure in place for a software developer to make use of the mechanism in a defined sense.
% Software developers wishing to adapt their code to use Intel SGX will manually adapt their code via annotations and apportionment of what computations will take place in a secure memory enclave that is implemented in hardware. 
% Here, we see that Intel SGX lends itself to a direct analysis of performance depreciation directly due to the use of Intel SGX by any party producing software applications.
% Due to Intel's unique position as one of only a few companies that dominates the design of computer CPUs, the Intel SGX mechanism is able to span the application stack, from the programmer level all the way down to the hardware level.
% Potential vendors on the software or hardware side of the spectrum are thus able to easily associate the use of the Intel SGX mechanism with a \textit{specific and measurable hit to performance}.

% This lies in contrast to the idea of a software-distributing vendor performing analysis on security improvements such as full system hardware-centered memory encryption. 
% We see that when we perform total memory encryption, we know that the data in our programs will be encrypted, but the full memory encryption mechanism has no ``knowledge" of what is being encrypted.
% This divide between the level of abstraction at which the mechanism has been implemented (hardware) and at which the programmer operates (application development) creates difficulties with respect to assigning some performance overhead to the use of the mechanism for that software developer.
% Because we would like the effort of the software vendor to adapt their software products for the use of a hardware mechanism such as full memory encryption, it must be necessary that the software vendor is able to describe the performance impact of their design decisions.
% We describe this type of security mechanism with the term \textit{diffuse}.
% A \textit{diffuse} security mechanism can be thought of as having its functionality distributed throughout the body of what it is securing.

% Practically, the difference between these two types of security mechanisms is the difficulty in assigning a meaningful measurement of a mechanism's performance overhead from the perspective of any vendor.
% If we require all vendors of hardware and software to give an accounting of how they are spending their security budget, it must be clear \textit{how} we would expect vendors to show that they are following the mandate meaningfully.
% In the case of a discrete mechanism, it is simple to show how to account for the impacts of the mechanism on performance metrics, but not so in the case of a diffuse mechanism.
% This is why we must show that in the case of a diffuse security mechanism, the burden of implementing our mandate is not heavy.
% We first give practical examples of existing discrete security mechanisms and show that they already lend themselves to accounting for the implementation of our mandate. 
% Then we explore the creation of a basic artificial neural network model that predicts performance overheads for some application given novel program inputs to the system, as an existence proof that it is not too much of a burden on the hardware or software side to account for the specific performance impact of using any potential security mechanism.











% Given the existence of a mandate as defined previously, we would like to analyze the burden of implementation.
% Ideally, the burden would be light and distributed in approximately equal proportions among the parties subject to such a mandate. We analyze the consequences of implementing our mandate in software or hardware and use the resulting conclusions to claim that in order to properly implement our mandate, we must modify the hardware-software interface, and thus the ISA.

% Ideally we'd like to know how much systems are spending toward security as a fraction of total performance. 
% To cohesively address why we conclude that our mandate becomes a problem of computer architecture, we first explore the concept of implementing the mandate in only software or hardware and see that these solutions ineffectively distribute the burden of implementation. We also back up these observations with case studies of real technologies viewed through the lens of being used to satisfy the security mandate that we propose.

Where a defense lies within this taxonomy determines how practical it is to apply towards a security-performance mandate.
Previously, diffuse and always-on defenses would be incompatible with such a mandate, since they require on-system benchmarking (explain further).
In the next section, we dramatically expand the number and types of defenses that can be considered for such a mandate by introducing a mechanism for determining on-system diffuse and continuous defenses.
